A Topological Application of Labelled Natural Deduction

We use a labelled deduction system based on the concept of computational paths (sequences of rewrites) as equalities between two terms of the same type. We also define a term rewriting system that is used to make computations between these computational paths, establishing equalities between equalities. We then proceed to show the main result here: using this system to obtain the calculation of the fundamental group of the circle, of the torus and the real projective plane.

==> glossaries.tex <==




\newglossaryentry{naive-bayes}
{
  name=\textit{Na{\"i}ve Bayes},
  description={},
  plural=\textit{Na{\"i}ve Bayes}
}

\newglossaryentry{hoeffding-tree}
{
  name=\textit{Hoeffding Tree},
  description={},
  plural=\textit{Hoeffding Trees}
}




\newglossaryentry{data-stream}
{
  name=\textit{Data Stream},
  description={},
  plural=\textit{Data Streams}
}


\newglossaryentry{single-detection-approach}
{
  name=\textit{Single Detection Approach},
  description={},
  plural=\textit{Single Detection Approachs}
}



\newglossaryentry{multiple-detection-approach}
{
  name=\textit{Multiple Detection Approach},
  description={},
  plural=\textit{Multiple Detection Approachs}
}

\newglossaryentry{single-detection}
{
  name=\textit{Single Detection},
  description={},
  plural=\textit{Single Detectors}
}


\newglossaryentry{single-detector}
{
  name=\textit{Single Detector},
  description={},
  plural=\textit{Single Detectors}
}



\newglossaryentry{multiple-classifier-system}
{
  name=\textit{Multiple classifier System},
  description={},
  plural=\textit{Multiple classifier Systems}
}
 

\newglossaryentry{prequential}
{
  name=\textit{Prequential},
  description={},
  plural=\textit{}
}


\newglossaryentry{single-classifier-base}
{
  name=\textit{Single Classifier-base},
  description={},
  plural=\textit{Single classifiers-base}
}

\newglossaryentry{multiple-processing-approach}
{
  name=\textit{Multiple Processing Approach},
  description={},
  plural=\textit{Multiple Processing Approachs}
}

\newglossaryentry{concept-drift}
{
  name=\textit{Concept Drift},
  description={},
  plural=\textit{Concept Drifts}
}


\newglossaryentry{multiple-detector}
{
  name=\textit{Multiples Detector},
  description={},
  plural=\textit{Multiples Detectors}
}

\newglossaryentry{single-detection-algorithm}
{
  name=\textit{Single Detection Algorithm},
  description={},
  plural=\textit{Single Detection Algorithms}
}

\newglossaryentry{ensemble-methods}
{
  name=\textit{Ensemble Methods},
  description={},
  plural=\textit{Ensembles Methods}
}












==> images/acronimos.tex <==


% CriaÃ§Ã£o de glossÃ¡rios e lista de abreviaÃ§Ãµes
%\usepackage[smallcaps}{glossaries}
\usepackage{amssymb}

\newacronym{zfc}{ZFC}{Zermelo-Frankel-Choice}
\newacronym{pif}{$\Pi - F$}{dependent function formation}
\newacronym{pii}{$\Pi - I$}{dependent function introduction}
\newacronym{pie}{$\Pi - E$}{dependent function elimination}
\newacronym{pic}{$\Pi - C$}{dependent function computation}
\newacronym{sif}{$\Sigma - F$}{dependent sum formation}
\newacronym{sii}{$\Sigma - I$}{dependent sum introduction}
\newacronym{sie1}{$\Sigma - E_{1}$}{first dependent sum elimination}
\newacronym{sie2}{$\Sigma - E_{2}$}{second dependent sum elimination}
\newacronym{sic}{$\Sigma - C$}{Computação da Soma Dependente}
\newacronym{n0}{$\mathbb N-I_{0}$}{zero introduction}
\newacronym{ns}{$\mathbb N-I_{s}$}{successor induction}
\newacronym{ifi}{$Id^{int} - I$}{identity type introduction}
\newacronym{iff}{$Id^{int} - F$}{identity type formation}
\newacronym{ie}{$Id - E$}{identity type elimination}
\newacronym{ii}{$Id - Eq$}{identity type equality}
\newacronym{ife}{$Id^{ext} - F$}{extensional identity type formation}
\newacronym{iie}{$Id^{ext} - I$}{extensional identity type introduction}
\newacronym{iee}{$Id^{ext} - E$}{extensional identity type elimination}
\newacronym{iei}{$Id^{ext} - Eq$}{extensional identity type equality}
\newacronym{bi}{$\lambda\beta\eta$}{Teoria da Beta-Eta Igualdade}
\newacronym{pf}{$\times - F$}{product formation}
\newacronym{pi}{$\times - I$}{product introduction}
\newacronym{pe1}{$\times - E_{1}$}{first product elimination}
\newacronym{pe2}{$\times - E_{2}$}{second product elimination}
\newacronym{rw}{$LND_{EQ}-TRS$}{Term Rewrite System}
\newacronym{uip}{UIP}{Uniqueness of Identity Proofs}
